Query Log Compression for Workload Analytics

Analyzing database access logs is a key part of performance tuning, intrusion detection, benchmark development, and many other database administration tasks. Unfortunately, it is common for production databases to deal with millions or even more queries each day, so these logs must be summarized before they can be used. Designing an appropriate summary encoding requires trading off between conciseness and information content. For example: simple workload sampling may miss rare, but high impact queries. In this paper, we present LogR, a lossy log compression scheme suitable use for many automated log analytics tools, as well as for human inspection. We formalize and analyze the space/fidelity trade-off in the context of a broader family of "pattern" and "pattern mixture" log encodings to which LogR belongs. We show through a series of experiments that LogR compressed encodings can be created efficiently, come with provable information-theoretic bounds on their accuracy, and outperform state-of-art log summarization strategies.

==> sections/0-abstract.tex <==
% !TEX root = ../paper.tex
\begin{abstract}
Database access logs are knowledge bases for many forms of database administration, from database performance tuning, to security auditing, to benchmark design, and many more. They record how the data was being used, combined, and/or manipulated in the history and support decision making(e.g. query recommendation, indexing etc) for the future. The knowledge can be captured from examining \textit{abstract syntax trees}(ASTs) of queries which encode \textit{correlation} among different data operations and ideally database administrators learns a distribution over all possible sub-trees of ASTs in the log. This distribution helps administrators seek sub-trees they might be interested(frequent, outlier, etc). Unfortunately, it is challenging for mining such distribution over large number of syntax tree structures. For scalability, these tree structures should be transformed into a structurally simpler \textit{representation}. However, for knowledge preserving, the original syntactic tree structures must be efficiently re-constructed by parsing the representation and it is non-trivial to balance between. In addition, when the database administrator is human, in order to prevent the human from being overwhelmed by the potentially huge number of parameters or \textit{verbosity} in the actual distribution, a succinct \textit{summary} distribution with reduced verbosity should be visualized instead. Parameter reduction inevitably makes summary deviates from the actual distribution and the definition of \textit{error} measuring such deviation should be properly designed and benchmarked. The trade-off curve of error versus verbosity should be measured and visualized from which the administrator can dynamically balance between. It is then crucial to `optimize' such curve by minimizing the summarization error under all possible verbosity levels. In this paper, we offer a systematic approach that addresses the series of mentioned challenging problems aimed at helping database administrators analyze database access logs fast, scalable and precise.
\end{abstract}

==> sections/5-datasets_methods.tex <==
% !TEX root = ../paper.tex




==> sections/5.5-system-overview.tex <==
% !TEX root = ../paper.tex

In this section, we introduce the log compression problem.








% In this section, we provide overview on a prototype system that interact with humans by presenting summarizes with controllable Summary Error versus Verbosity.
% \subsection{System Architecture}
% We start by showing the interaction between different system components in Figure~\ref{fig:systemoverview}.
% \begin{figure}[h!]
% \includegraphics[width=0.5\textwidth]{graphics/System_Overview.pdf}
% \centering
% \caption{Prototype System Architecture}
% \label{fig:systemoverview}
% \end{figure}

% \subsection{Example Output}


% \subsection{System Applications}

